Synbit: Synthesizing Bidirectional Programs using Unidirectional Sketches

We propose a technique for synthesizing bidirectional programs from the corresponding unidirectional code plus a few input/output examples. The core ideas are: (1) constructing a sketch using the given unidirectional program as a specification, and (2) filling the sketch in a modular fashion by exploiting the properties of bidirectional programs. These ideas are enabled by our choice of programming language, HOBiT, which is specifically designed to maintain the unidirectional program structure in bidirectional programming, and keep the parts that control bidirectional behavior modular. To evaluate our approach, we implemented it in a tool called Synbit and used it to generate bidirectional programs for intricate microbenchmarks, as well as for a few larger, more realistic problems. We also compared Synbit to a state-of-the-art unidirectional synthesis tool on the task of synthesizing backward computations.

==> implementation.tex <==
\section{Implementation}


% We implemented our procedure in Haskell.
% The implementation can be seen in \url{https://github.com/masaomi-yamaguchi/Masaomi-Yamaguchi-Master-Thesis}.

This section reports our prototype implementation of the proposed synthesis method, which is
available in \url{https://github.com/masaomi-yamaguchi/synbit}.

The prototype system is implemented in Haskell as an extension to the original prototype implementation of HOBiT by Matsuda,\footnote{\url{https://bitbucket.org/kztk/hibx/}}
which also uses Haskell.
As we have mentioned in the previous section, our synthesis method utilizes the lazy nondeterministic generation.
For this step, the prototype implementation uses a variant of \citet{DBLP:journals/jfp/FischerKS11}'s library that implements Curry-like nondeterministic computation in Haskell,
with an extension with weights on nondeterministic choices, which serve as priorities in searching.
Basically, a choice to increase the program size has a positive weight so that smaller programs have higher priorities in searching.

% Our procedure is based on the generate-and-test approach. To do generate-and-test efficiently, we use a method for lazy non-deterministic programming in Haskell \cite{DBLP:journals/jfp/FischerKS11} like Curry. By using this method, we can delay generation until it is needed.
% We extended the method \cite{DBLP:journals/jfp/FischerKS11} naturally to use priority for searching.


==> kztk_macro.tex <==
\makeatletter
\def\qedmath{%
   \relax\ifmmode
      \@badmath
   \else
      \begin{trivlist}%
         \@beginparpenalty\predisplaypenalty
         \@endparpenalty\postdisplaypenalty
         \item[]\leavevmode
         \hbox to\linewidth\bgroup\relax\hfil$\displaystyle
            \bgroup
            \fi
            }
            \def\endqedmath{%
            \relax\ifmmode
            \egroup $\hfil \egroup\\[-\baselineskip]
         \hbox{}\hfill\llap{\phantom{0}\qed}
      \end{trivlist}
   \else
      \@badmath
   \fi
}
\def\qedflmath{\relax \ifmmode \@badmath
   \else\begin{trivlist}%
         \@beginparpenalty\predisplaypenalty
         \@endparpenalty\postdisplaypenalty
         \item[]\leavevmode \hb@xt@\linewidth\bgroup $\m@th\displaystyle %$
            \hskip\mathindent\bgroup
            \fi}
            \def\endqedflmath{\relax\ifmmode
            \egroup $% $
         \egroup \\[-\baselineskip]\hskip\linewidth\llap{\qed}
      \end{trivlist}%
   \else \@badmath
   \fi}
\makeatother

\newcommand{\todo}[1]{\textcolor{red}{\textbf{[TODO: #1]}}}
%\newcommand{\todo}[1]{}
\newcommand{\kztk}[1]{\textcolor{blue}{[kztk: #1]}}
\newcommand{\meng}[1]{\textcolor{green}{[Meng: #1]}}
\newcommand{\masaomi}[1]{\textcolor{magenta}{[masaomi: #1]}}
\definecolor{gold}{RGB}{218,165,32}


\newcommand{\mi}[1]{\ensuremath{\mathit{#1}}}
\newcommand{\mr}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\ms}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\mt}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}}

\newcommand{\foreignWord}[1]{#1}
% \newcommand{\eg}{\foreignWord{e.g.}\xspace}
% \newcommand{\ie}{\foreignWord{i.e.}\xspace}
% \newcommand{\cf}{\foreignWord{cf.}\xspace}
% \newcommand{\etal}{\foreignWord{et al.}\xspace}
% \newcommand{\wrt}{{w.r.t.}\xspace}

% Since the List of Accepted LaTeX Packages (insanely) does not
% contain xspace, so these macros should be used as `\eg{}` for
% example.
\newcommand{\eg}{\foreignWord{e.g.}}
\newcommand{\ie}{\foreignWord{i.e.}}
\newcommand{\cf}{\foreignWord{cf.}}
\newcommand{\etal}{\foreignWord{et al.}}
\newcommand{\wrt}{{w.r.t.}}


% Greek letters

\newcommand{\Gl}{\lambda}
\newcommand{\Ga}{\alpha}
\newcommand{\Gb}{\beta}
\newcommand{\Gk}{\kappa}
\newcommand{\Gr}{\rho}
\newcommand{\Gs}{\sigma}
\newcommand{\GS}{\Sigma}
\newcommand{\Gt}{\tau}
\newcommand{\Gth}{\theta}
\newcommand{\GTH}{\Theta}
\newcommand{\GTh}{\Theta}
\newcommand{\Gg}{\gamma}
\newcommand{\GG}{\Gamma}
\newcommand{\Gd}{\delta}
\newcommand{\GD}{\Delta}

\newcommand{\x}{\times}
\newcommand{\ox}{\otimes}

\newenvironment{tarray}[2][c]{%
\settowidth{\dimen1}{${} = {}$}%
   \setlength{\arraycolsep}{0.125\dimen1}
   \hspace{-0.125\dimen1}\array[#1]{#2}\relax
}
{%
   \endarray\hspace{-0.125\dimen1}
}
\newcommand{\bb}{\tarray{lllll}}
\newcommand{\bbc}{\tarray{c}}
\newcommand{\bbt}{\tarray[t]{lllll}}
\newcommand{\bbb}{\tarray[b]{lllll}}
\newcommand{\ee}{\endtarray}

\newcommand{\from}{\leftarrow}
\newcommand{\To}[0]{\Rightarrow}
\newcommand{\From}{\Leftarrow}

\newcommand{\bba}{\alignedat{8}}
\newcommand{\bbat}{\alignedat[t]{8}}
\newcommand{\eea}{\endalignedat}

\newcommand{\APPEND}{\mathbin{+\!+}}

\newcommand{\DOLLAR}{\ensuremath{\mathbin{\texttt{\$}}}}
\newcommand{\key}[1]{\ensuremath{\mathbf{#1}}} % keyword
\newcommand{\api}[1]{\ensuremath{\mathsf{#1}}} % api

\newcommand{\DATA}{\key{data}}
\newcommand{\TYPE}{\key{type}}
\newcommand{\WHERE}{\key{where}}
\newcommand{\CASE}{\key{case}}
\newcommand{\CASEEX}[3]{\CASE~#1~\OF #2 \bbt #3 \ee}

\newcommand{\WITH}{\key{with}}
\newcommand{\RECONCILED}{\key{reconciled}}
\newcommand{\BY}{\key{by}}
\newcommand{\OF}{\key{of}}
\newcommand{\DO}{\key{do}}
\newcommand{\LET}{\key{let}}
\newcommand{\IN}{\key{in}}

\newcommand{\dontcare}{%
   \settowidth{\dimen2}{v}%
   \hspace{0.05\dimen2}\rule{0.9\dimen2}{0.5pt}\hspace{0.05\dimen2}}
\newcommand{\A}{\;}

\newcommand{\IF}{\key{if}}
\newcommand{\THEN}{\key{then}}
\newcommand{\ELSE}{\key{else}}
\newcommand{\shortequals}{%
   {\rlap{\rule[0.14em]{.25em}{0.5pt}}{\rule[0.34em]{.25em}{0.5pt}}}
}

\newcommand{\doubleequals}{\ensuremath{\mathrel{%
         \shortequals\,\shortequals}}}
\newcommand{\ndoubleequals}{%
   \ensuremath{\not\expandafter\doubleequals}}

\newcommand{\LCOMMENT}[1]{\texttt{-{}-}~\text{#1}}
\newcommand{\COMMENT}[1]{\texttt{\{-}~\text{#1}~\texttt{-\}}}

\makeatletter
\newcounter{pe@nocounter}
\newcommand{\peano}[1]{%
   \setcounter{pe@nocounter}{#1}
   \pe@no}
\newcommand{\pe@no}{%
   \ifnum\value{pe@nocounter}>1
      \addtocounter{pe@nocounter}{-1}%
      \con{S} \A (\expandafter\pe@no)%
   \else%
      \ifnum\value{pe@nocounter}>0%
         \con{S} \A \con{Z}%
      \else%
         \con{Z}%
      \fi%
   \fi%
}

\newcommand{\con}[1]{\ms{#1}}
\newcommand{\var}[1]{\mi{#1}}

\newcommand{\str}[1]{\texttt{"#1"}}
\newcommand{\chr}[1]{\texttt{'#1'}}

\newcommand{\lub}{\curlyvee}

\newcommand{\V}[1]{\overline{#1}}
\newcommand{\Size}[1]{\lvert{#1}\rvert}

\newcommand{\fv}{\mathrm{fv}}
\newcommand{\dom}{\mathrm{dom}}

\definecolor{bxcolor}{rgb}{0.05,0.15,0.76}

\makeatletter
\newif\ifbxgrayed@ut
\newcommand{\grayout}{\bxgrayed@uttrue\color{gray}}
\newcommand{\grayoutend}{\bxgrayed@utfalse}

\newcommand{\bxcolor}{\ifbxgrayed@ut\color{gray}\else\color{bxcolor}\fi}
\newcommand{\textbxcolor}[1]{\ifbxgrayed@ut\textcolor{gray}{#1}\else\textcolor{bxcolor}{#1}\fi}

\newcommand{\bx}[1]{{\bxcolor\underline{#1}}}
\newcommand{\BX}[1]{{\bxcolor\mathbf{B}{#1}}}
\newcommand{\LIFTU}[1]{{{\bxcolor!}#1}}

\makeatother

\newcommand{\bxkey}[1]{\bx{\key{#1}}}
\newcommand{\bxcon}[1]{\bx{\con{#1}}}
\newcommand{\bxop}[1]{\mathbin{\bx{#1}}}

\newcommand{\bxtup}[1]{\bx{(}#1\bx{)}}

\newcommand{\BCASE}{\bxkey{case}}
\newcommand{\BLET}{\bxkey{let}}
\newcommand{\BIN}{\bxkey{in}}
\newcommand{\BOF}{\bxkey{of}}
\newcommand{\BWITH}{\bxkey{with}}
\newcommand{\BBY}{\bxkey{by}}


\newcommand{\infer}[2]{\frac{\displaystyle#2}{\displaystyle#1}}
\newcommand{\ninfer}[3]{\infer{#2}{#3}\,\text{(\rname{#1})}}
\newcommand{\rname}[1]{\textsc{#1}}

\newcommand{\GET}{\mathit{get}}
\newcommand{\PUT}{\mathit{put}}

\newcommand{\evalU}{\Downarrow}
\newcommand{\evalB}{\Leftarrow}
\newcommand{\evalF}{\Rightarrow}

\newcommand{\EvalRelU}[2]{#1 \evalU #2}
\newcommand{\EvalRelF}[3]{#1 \vdash_\mathrm{G} #2 \evalF #3}
\newcommand{\EvalRelB}[4]{#1 \vdash_\mathrm{P} #2 \evalB #3 \dashv #4}

\newcommand{\sem}[1]{\llbracket#1\rrbracket}

\newcommand{\ExSet}{\mathcal{E}}


==> synthesis/type.tex <==
\subsubsection{Synthesize the Types of the Functions}\label{sec:synthesis-type}

In the first step, our procedure enumerates all candidates for types of bidirectionalied functions.
We obtain candidates for types of functions by adding $\BX{}$ to some part of the type of the given unidirectional program.
The type of the entry point $f_1$ is already fixed as $\BX{\sigma_1}\to \BX{\tau_0}$.
To take consistency between types of functions, enumerate all candidate for types of $f_2\ldots f_n$.
You may think that it is enough to add $\BX{}$ before and behind $\to$ as with $f_1$ (e.g. convert $\con{Int} \to \con{Int} \to \con{Int}$ into $\BX{\con{Int}} \to \BX{\con{Int}} \to \BX{\con{Int}}$), however, it is not good way.
$\var{appendBc} :: \BX{[a]} \to [a] \to \BX{[a]}$ in section \ref{sec:prelim} is a good example.
Since the second argument is not $\BX{}$, we can use it in the with condition. If the type of the second argument is $\BX{}$, we cannot write such a with condition.
Thus, we cannot find whether $\BX{}$ should be added only based on types.

The non-deterministic rules for generating types $\mathcal{B}(A)$ is given in figure \ref{fig:synthesis-type}.
We omit $\to$ and $\BX{}$ in $\BX{}$ for HOBiT's restriction, although it is not written in rules.
\begin{figure}[t]
  \setlength{\abovedisplayskip}{0pt}
  \setlength{\belowdisplayskip}{0pt}
  \begin{alignat*}{6}
     & \mathcal{B}(\con{Bool})            &  & \leadsto & \  & \con{Bool}                                  & \qquad & \mathcal{B}(\con{Bool}) &  & \leadsto & \  & \BX{\con{Bool}} \\
     & \mathcal{B}([\tau])                &  & \leadsto & \  & [\mathcal{B}(\tau)]                         & \qquad & \mathcal{B}([\tau])     &  & \leadsto & \  & \BX{[\tau]}     \\
     & \mathcal{B}(\rm \tau_1 \to \tau_2) &  & \leadsto & \  & \mathcal{B}(\tau_1) \to \mathcal{B}(\tau_2)
  \end{alignat*}
  \caption{Generation of Candidates for Types : $\mathcal{B}(A)$}
  \label{fig:synthesis-type}
\end{figure}
The algorithm for converting the type environment $\Gamma'_\mathrm{in}$ into the $\BX{}$\nobreakdash-type environment $\Gamma'_\mathrm{in}$ is shown in figure \ref{fig:algo-synthesis-type}.
\begin{figure}[t]
  \setlength{\abovedisplayskip}{0pt}
  \setlength{\belowdisplayskip}{0pt}
  % \begin{tabular}{lp{10cm}}
  %   \textbf{Input}     & $\Gamma_\mathrm{in}=\{f_1:\sigma _1\to \tau_1\}\uplus \{f_i:F_i\}_{i\in\{2\ldots n\}}$ \\
  %   \textbf{Output}    & $\Gamma'_\mathrm{in}=\{f_i:F_i'\}_{i\in\{1\ldots n\}}$                                         \\
  %   \textbf{Procedure} & \vspace{-0.5em}\begin{enumerate}
  %     \item Let $F_1':=\forall \BX{\sigma_1}\to \BX{\tau_1}$.
  %     \item Calculate $\mathcal{B}(F_i)\leadsto F_i'$ nondeterministically for all $i\in\{2\ldots n\}$.
  %     \item Return $\{f_i:F_i'\}_{i\in\{1\ldots n\}}$.
  %   \end{enumerate}
  % \end{tabular}
  \begin{description}
    \item[Input]\ \ \,$\Gamma_\mathrm{in}=\{f_1:\sigma _1\to \tau_1\}\uplus \{f_i:F_i\}_{i\in\{2\ldots n\}}$
    \item[Output]$\Gamma'_\mathrm{in}=\{f_i:F_i'\}_{i\in\{1\ldots n\}}$
    \item[Procedure]\
          \begin{enumerate}
            \item Let $F_1':=\BX{\sigma_1}\to \BX{\tau_1}$.
            \item Calculate $\mathcal{B}(F_i)\leadsto F_i'$ nondeterministically for all $i\in\{2\ldots n\}$.
            \item Return $\{f_i:F_i'\}_{i\in\{1\ldots n\}}$.
          \end{enumerate}
  \end{description}
  \caption{Algorithm: Generation of Candidates for Type Environment}
  \label{fig:algo-synthesis-type}
\end{figure}

\begin{example}(Type Candidates for Bidirectional $\var{append}$)\label{ex:append-type-candidates}
  The type of bidirectional $\var{appendPair}$ is fixed as $\BX{([\con{Int}],[\con{Int}])} \to \BX{[\con{Int}]}$.
  The type
  $[\con{Int}]\to[\con{Int}]\to[\con{Int}]$, which is the type of $\var{append}$, is converted nondeterministically as follows:
  {\footnotesize
  % use [lll] in matrix
  \makeatletter
  \renewcommand*\env@matrix[1][*\c@MaxMatrixCols c]{%
    \hskip -\arraycolsep
    \let\@ifnextchar\new@ifnextchar
    \array{#1}}
  \makeatother
  \begin{align*}
     & \mathcal{B}([\con{Int}]\to[\con{Int}]\to[\con{Int}]) \\
     & \leadsto \left\{\begin{matrix}[lll]
      [\con{Int}] \to [\con{Int}] \to [\con{Int}]       ,     & [\con{Int}] \to [\con{Int}] \to [\BX{\con{Int}}]       ,     & [\con{Int}] \to [\con{Int}] \to \BX{[\con{Int}]}       ,     \\
      [\con{Int}] \to [\BX{\con{Int}}] \to [\con{Int}]    ,   & [\con{Int}] \to [\BX{\con{Int}}] \to [\BX{\con{Int}}]    ,   & [\con{Int}] \to [\BX{\con{Int}}] \to \BX{[\con{Int}]}    ,   \\
      [\con{Int}] \to \BX[\con{Int}] \to [\con{Int}]     ,    & [\con{Int}] \to \BX[\con{Int}] \to [\BX{\con{Int}}]     ,    & [\con{Int}] \to \BX[\con{Int}] \to \BX{[\con{Int}]}     ,    \\
      [\BX{\con{Int}}] \to [\con{Int}] \to [\con{Int}]    ,   & [\BX{\con{Int}}] \to [\con{Int}] \to [\BX{\con{Int}}]    ,   & [\BX{\con{Int}}] \to [\con{Int}] \to \BX{[\con{Int}]}    ,   \\
      [\BX{\con{Int}}] \to [\BX{\con{Int}}] \to [\con{Int}] , & [\BX{\con{Int}}] \to [\BX{\con{Int}}] \to [\BX{\con{Int}}] , & [\BX{\con{Int}}] \to [\BX{\con{Int}}] \to \BX{[\con{Int}]} , \\
      [\BX{\con{Int}}] \to \BX[\con{Int}] \to [\con{Int}]  ,  & [\BX{\con{Int}}] \to \BX[\con{Int}] \to [\BX{\con{Int}}]  ,  & [\BX{\con{Int}}] \to \BX[\con{Int}] \to \BX{[\con{Int}]}  ,  \\
      \BX{[\con{Int}]} \to [\con{Int}] \to [\con{Int}]    ,   & \BX{[\con{Int}]} \to [\con{Int}] \to [\BX{\con{Int}}]    ,   & \BX{[\con{Int}]} \to [\con{Int}] \to \BX{[\con{Int}]}    ,   \\
      \BX{[\con{Int}]} \to [\BX{\con{Int}}] \to [\con{Int}] , & \BX{[\con{Int}]} \to [\BX{\con{Int}}] \to [\BX{\con{Int}}] , & \BX{[\con{Int}]} \to [\BX{\con{Int}}] \to \BX{[\con{Int}]} , \\
      \BX{[\con{Int}]} \to \BX[\con{Int}] \to [\con{Int}]  ,  & \BX{[\con{Int}]} \to \BX[\con{Int}] \to [\BX{\con{Int}}]  ,  & \BX{[\con{Int}]} \to \BX[\con{Int}] \to \BX{[\con{Int}]}
    \end{matrix}
    \right\}
  \end{align*}}
\end{example}

